Automatic Face Understanding: Recognizing Families in Photos

We built the largest database for kinship recognition. The data were labeled using a novel clustering algorithm that used label proposals as side information to guide more accurate clusters. Great savings in time and human input was had. Statistically, FIW shows enormous gains over its predecessors. We have several benchmarks in kinship verification, family classification, tri-subject verification, and large-scale search and retrieval. We also trained CNNs on FIW and deployed the model on the renowned KinWild I and II to gain SOTA. Most recently, we further augmented FIW with MM. Now, video dynamics, audio, and text captions can be used in the decision making of kinship recognition systems. We expect FIW will significantly impact research and reality. Additionally, we tackled the classic problem of facial landmark localization. A majority of these networks have objectives based on L1 or L2 norms, which inherit several disadvantages. The locations of landmarks are determined from generated heatmaps from which predicted landmark locations get penalized without accounting for the spread: a high scatter corresponds to low confidence and vice-versa. To address this, we introduced an objective that penalizes for low confidence. Another issue is a dependency on labeled data, which is expensive to collect and susceptible to error. We addressed both issues by proposing an adversarial training framework that leverages unlabeled data to improve model performance. Our method claims SOTA on renowned benchmarks. Furthermore, our model is robust with a reduced size: 1/8 the number of channels is comparable to SOTA in real-time on a CPU. Finally, we built BFW to serve as a proxy to measure bias across ethnicity and gender subgroups, allowing us to characterize FR performances per subgroup. We show performances are non-optimal when a single threshold is used to determine whether sample pairs are genuine.

==> Makefile <==
# ------------------------------------------------------------------------
# Makefile:
# ------------------------------------------------------------------------
# written by:	Gunar Schirner 
# External References:
#   http://kriemhild.uft.uni-bremen.de/viewvc/vim/Makefile.pdflatex
#   http://www.tex.ac.uk/tex-archive/help/uk-tex-faq/Makefile
# last update:	$id$
#
# Help screen (start every help line with #h)
#
#h make        builds ALL_REF
#h
#h make publish 
#h             publish the build output to HTML publish directory  
#h
# --- names --------------------------------------------------------------

PROJECT	=	thesis

SRCNAME	=	$(PROJECT)_SRC.tar.gz
BINNAME	=	$(PROJECT)_BIN.tar.gz
ORIG	=	

TMP	=	/tmp
# own name
MAKEF   =       Makefile

# path for automatic publishing, put into your public_html directory`
PUBLISH_PATH = /home/student/<studentName>/public_html/thesis
VERSION_FILE = svnRev.tex

# set automatically by hook script (Post commit hook)
# SVN_REPO_PATH 
# SVN_REV

# --- lists --------------------------------------------------------------

ALL	=	$(PROJECT).pdf



# auto use all *.tex file in the own and in pi directory as dependency input 
INCLUDE	:=	$(shell [ -d tex ] && echo tex/*.tex )

SOURCES =	$(PROJECT).tex	\
		$(INCLUDE)

#BIBFILES :=  macro/bib-strings.bib macro/IEEEabrv.bib $(shell [ -d bib ] && echo bib/*.bib )

FIGFILES =

PPTFILES =	

PRNFILES =

# auto use all *.eps files in the fig directory as a dependency input 
#  FIGURES directory may not exist
# uncomment once first eps is added 
EPSFILES :=	$(shell [ -d fig ] && echo fig/*.eps) 


# auto use all *.pdf files in the fig directory as a dependency input 
#  FIGURES directory may not exist
# uncomment once first pdf is added 
#PDFFIGS :=	$(shell [ -d fig ] && echo fig/*.pdf) 


FIGURES	=	$(EPSFILES:.eps=.pdf) $(PDFFIGS)

#MACROS	=	macro/macros.tex

OTHERS	=	Makefile	


ORIGS	=	$(SOURCES) $(MACROS) $(OTHERS)

SRCTAR	=	$(SOURCES) $(MACROS) $(OTHERS)	\
		$(FIGFILES) $(PPTFILES) $(PRNFILES) $(EPSFILES)

BINTAR	=	$(ALL)

# --- environment --------------------------------------------------------

TEXINPUTS =	TEXINPUTS=.:MACROS:

TEXENV	=	$(TEXINPUTS)

# --- commands -----------------------------------------------------------

FIGPS	=	fig2dev -L ps
PRN2EPS	=	PATH=bin:$$PATH prn2eps
LATEX	=	$(TEXENV) latex
PDFLATEX =      pdflatex --interaction nonstopmode
BIBTEX	=	bibtex
DVIPS	=	dvips -Z -D 600 -t letter -Ppdf
PS2PDF	=	ps2pdf
EPS2PDF	=	epstopdf
PSSEL	=	psselect
TAR	=	gtar cvzf
RM	=	rm -f
MV	=	mv -f
MAKEIDX	=	makeindex
GV	=	ghostview
ECHO	=	echo
GREP	=	grep
WC	=	wc
CD	=	cd
CAT	=	cat
XLESS	=	xless
SPELL	=	nspell -t
SORT	=	sort -f
MAKEIDX	=	makeindex
DISTILL =       GS_OPTIONS="-dAutoFilterColorImages=false \
                            -dColorImageFilter=/FlateEncode" ps2pdf14
THUMBPDF=       thumbpdf --modes=dvips

# parse string to cause rebuild of latex
RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right|Table widths have changed. Rerun LaTeX.|Linenumber reference failed)"

# parse string to cause rebuild of bibtex
RERUNBIB = "No file.*\.bbl|Citation.*undefined"



# --- general rules ------------------------------------------------------

.SUFFIXES:
.SUFFIXES:	.fig .ps .prn .eps .tex .bbl .pdf

.fig.ps:
	$(FIGPS) $*.fig $*.ps

.prn.eps:
	$(PRN2EPS) $*.prn $*.eps

#GS added automatic conversion for eps files, epstopdf packages seems
# not installed on this linux installation
.eps.pdf:
	$(EPS2PDF) $*.eps

.tex.bbl:
	$(LATEX) $*.tex
	$(BIBTEX) $*

# run pdflatex once and bib + subsequent pdflatex conditionally
%.pdf: %.tex
	$(PDFLATEX) $<
	@egrep -c $(RERUNBIB) $*.log && (bibtex $*;$(PDFLATEX) $<); true
	@egrep $(RERUN) $*.log && ($(PDFLATEX) $<) ; true
	@egrep $(RERUN) $*.log && ($(PDFLATEX) $<) ; true


# --- rules --------------------------------------------------------------

all:		$(ALL)

# automatically produce help message by grep for sepcial comment lines 
help:;	@sed -n -e 's/^#h//p'  < $(MAKEF) | sed -e 's/ALL_REF/$(ALL)/g'

# second phase of the publish requires to get the current SVN version 
ifdef SECOND_PHASE
SVN_REV := $(shell svn info | sed -n -e 's/.*Revision: //p')
endif

# debug rule to print current version 
echo_ver:
	@echo $(SVN_REV)

# paste the current version information into tex file so that it 
# can be included into build
create_version_file: 
	@echo "\\newcommand{\\svnRevRef}{$(SVN_REV)}" > $(VERSION_FILE)


# actual publishing action 
autobuild_publish_2nd: create_version_file
	make >  $(PUBLISH_PATH)/z_buildlog.r$(SVN_REV).log
	set -e ; for f in $(basename $(filter %.pdf, $(ALL))); do        \
		rm -f $(PUBLISH_PATH)/$$f.r*.pdf;                         \
		cp $$f.pdf $(PUBLISH_PATH)/$$f.r$(SVN_REV).pdf;   \
		rm -f $(PUBLISH_PATH)/$$f.pdf; \
		ln -s $(PUBLISH_PATH)/$$f.r$(SVN_REV).pdf $(PUBLISH_PATH)/$$f.pdf ;  \
	done

# if the revision is already passed in as a parameter, we do not 
# need to trieve it again 
ifneq ("$(SVN_REV)", "")
# clean update build and publish 
publish: clean svn_up autobuild_publish_2nd
else
# cleanup, svn update and kick off second phase
publish: 
	make clean
	svn up
	make autobuild_publish_2nd SECOND_PHASE=1
endif

# helper rule to call svn update 
svn_up: 
	svn up


clean:
	$(RM) $(ALL)
	$(RM) *.ps *.pdf
	$(RM) *.dvi
	$(RM) *.toc *.lot *.lof *.log *.aux
	$(RM) *.idx *.ind *.ilg
	$(RM) *.inx *.srt
	$(RM) *.blg *.bbl
	$(RM) *.out
	$(RM) *.BAK *.bak *~
	$(RM) macro/*.BAK macro/*.bak macro/*~
	$(RM) texput.log
	$(RM) $(ORIG)

tar:
	-$(MV) $(SRCNAME) $(SRCNAME).bak
	-$(MV) $(BINNAME) $(BINNAME).bak
	-$(TAR) $(SRCNAME) $(SRCTAR)
	-$(TAR) $(BINNAME) $(BINTAR)

spell:
	$(SPELL) $(SOURCES)

orig:	$(ORIG)

todo:	$(ORIG)
	-$(GREP) -n "\.\.\.\." `$(CAT) $(ORIG)` >$(TMP)/todo
	$(WC) -l $(TMP)/todo ; $(XLESS) $(TMP)/todo ; $(RM) $(TMP)/todo &

1:
	$(LATEX) $(PROJECT).tex
	$(DVIPS) $(PROJECT).dvi -o $(PROJECT).ps

2:
	$(LATEX) $(PROJECT).tex
	$(LATEX) $(PROJECT).tex
	$(DVIPS) $(PROJECT).dvi -o $(PROJECT).ps


# --- project rules ---

$(PROJECT).pdf:  $(PROJECT).tex $(MACROS) $(INCLUDE) $(FIGURES) $(BIBFILES) 


summary.pdf:	summary.tex

$(PROJECT).ps: $(PROJECT).pdf
	pdf2ps $<

Description.ps: $(PROJECT).ps
	$(PSSEL) 1-15 $(PROJECT).ps Description.ps

Description.pdf:	Description.ps
	$(DISTILL) Description.ps Description.pdf


References.ps: $(PROJECT).ps
	$(PSSEL) 16- $(PROJECT).ps References.ps

References.pdf:	References.ps
	$(DISTILL) References.ps References.pdf


# --- other rules ---

$(ORIG):	$(ORIGS)
	$(ECHO) >$(ORIG) $(ORIGS)



#h dbgPrint   VAR=<varName> print content of variable <varName>
dbgPrint:
	@echo "$(VAR)=$($(VAR))"
# --- EOF ----------------------------------------------------------------


==> tables/dbtables.tex <==
    
    
    \begin{tabular}{>{\raggedleft}p{.45in}|>{\centering}p{.25in}|>{\centering}p{1.4in}|>{\centering}p{1.4in}|p{1.7in}|>{\raggedright\arraybackslash}p{2.0in}}
    \toprule
        DB& Ref(s)& Stats & Label types & Metric, performance, \ac{sota} & Web\tabularnewline\midrule
        \multirow{2}{*}{CornellKin} 
        &\multirow{2}{*}{\cite{fang2010towards}}& \multirow{2}{*}{\textbullet~150~\textbf{F} \textbullet~300~\textbf{S} \textbullet~300~\textbf{f}} &\multirow{2}{*}{parent-child} &\multirow{2}{*}{verification accuracy  94.4\%~\cite{kohli2018supervised}} & \href{http://chenlab.ece.cornell.edu/projects/KinshipVerification/}{http://chenlab.ece.cornell.edu/ projects/KinshipVerification/}\tabularnewline \midrule
        
        \multirow{2}{*}{UB Face} &\cite{shao2011genealogical}~\cite{Xia201144}& \multirow{2}{*}{\textbullet~200~\textbf{F} \textbullet~250~\textbf{P} \textbullet~600~\textbf{f} \textbullet~400~\textbf{S}}& \multirow{2}{*}{[young, old] parent-child} &\multirow{2}{*}{accuracy, 95.3\%~\cite{kohli2018supervised}} &  \href{http://www1.ece.neu.edu/~yunfu/research/Kinface/Kinface.htm}{http://www1.ece.neu.edu/yunfu/ research/Kinface/}\tabularnewline
        \midrule
        
        \multirow{2}{*}{Twins Day} &  \multirow{2}{*}{\cite{vijayan2011twins}}& \textbullet~1,736~(finger, 3D face, iris, DNA)~\textbf{S} \textbullet~197~\textbf{I} & \multirow{2}{*}{Twin pairs}& \multirow{2}{*}{accuracy, 98.8\%~\cite{vijayan2011twins}}& \href{https://biic.wvu.edu/data-sets/twins-day-dataset-2010-1015}{/twins-day-dataset-2010-1015}\tabularnewline\midrule
    
        \multirow{2}{*}{SibFace} & \cite{bottino2012new} &\multirow{2}{*}{\textbullet~184~\textbf{S} \textbullet~78~\textbf{P} \textbullet~78~\textbf{F} \textbullet~184~\textbf{f}}& siblings (brothers, sisters, mixed)&\multirow{2}{*}{accuracy, 52.5\%~\cite{guo2014graph}}&
       \href{https://areeweb.polito.it/ricerca/cgvg/siblingsDB.html}{https://areeweb.polito.it/ricerca/ cgvg/siblingsDB.html}\tabularnewline\midrule
        
        \multirow{2}{*}{Family101} &\multirow{2}{*}{\cite{fang2013kinship}} &\multirow{2}{*}{\textbullet~101~\textbf{F} \textbullet~607~\textbf{S}}& \multirow{2}{*}{Family-tree structure}&  \multirow{2}{*}{Rank@10, 70.1\%~\cite{wu2018kinship}}& \href{http://chenlab.ece.cornell.edu/projects/KinshipClassification/index.html}{http://chenlab.ece.cornell.edu/ projects/KinshipClassification/}\tabularnewline\midrule

        \multirow{2}{*}{KFW I + II} &\multirow{2}{*}{\cite{lu2015fg}}&\textbullet~533 + 1,000~\textbf{P} \textbullet~1,066 + 2,000~\textbf{f} & parent-child; same + different photo& \multirow{2}{*}{accuracy, 96.9\% + 97.1\%~\cite{kohli2018supervised}} &\multirow{2}{*}{\href{http://www.kinfacew.com/}{http://www.kinfacew.com/}}\tabularnewline\midrule

        \multirow{1}{*}{TSKin} &  \multirow{1}{*}{\cite{qin2015tri}}&\multirow{1}{*}{\textbullet~787~\textbf{F} \textbullet~2,589~\textbf{S}} &\multirow{1}{*}{father/mother-child}& \multirow{1}{*}{accuracy, 91.4\%~\cite{liang2018weighted}}&
        \href{http://parnec.nuaa.edu.cn/xtan/data/TSKinFace.html}{parnec.nuaa.edu.cn/TSKinFace} \tabularnewline\midrule
    
    
        \multirow{2}{*}{FIW}& \cite{robinson2016families, wang2017kinship, robinson2018visual, robinson2020recognizing} &\textbullet~1,000~\textbf{F} \textbullet~33,000~\textbf{f} \textbullet~1-M~\textbf{P} \textbullet12,000~\textbf{S} \textbullet~13,000~\textbf{I} &large-scale; person-, family-, \& image-level.& accuracy, 78\%; tri-verification accuracy, 79\%; mAP 18\% \& Rank@5 60\%~\cite{robinson2020recognizing} &\href{https://web.northeastern.edu/smilelab/fiw/}{https://web.northeastern.edu/} \href{https://web.northeastern.edu/smilelab/fiw/}{smilelab/fiw/}\tabularnewline\midrule
        
        \multirow{2}{*}{KFVW} &\multirow{2}{*}{\cite{yan2018video}} & \textbullet~418 (video) \textbf{P} (100-500 \textbf{f} per video);&  \multirow{2}{*}{father/mother-son/daugther} &
         \multirow{2}{*}{accuracy, 61.8\%~\cite{yan2018video}}& \multirow{2}{*}{\href{https://www.kinfacew.com/index.html}{https://www.kinfacew.com}}\tabularnewline\midrule
        
        
        \multirow{2}{*}{KIVI} &    \multirow{2}{*}{\cite{kohli2018supervised}} & \multirow{2}{*}{\textbullet~503 (video) \textbf{S} \textbullet~503 \textbf{I}} & \multirow{2}{*}{7 relationships (core family)} &   \multirow{2}{*}{accuracy, 83.2\%~\cite{kohli2018supervised}} & \href{http://iab-rubric.org/resources/KIVI.html}{http://iab-rubric.org/resources/KIVI.html} \tabularnewline
        % \midrule
        
    %     TALKIN &~\cite{wu2019audio}  &\textbullet~400 (video \& audio)~\textbf{P}&{parent-child}& accuracy, 74.1\% 
    %   \\
        % \bottomrule
    \end{tabular}

==> tables/results_table.tex <==

% \begin{table}[t!]
% \centering

% \centering
% % \vspace{8pt}
% % \resizebox{\linewidth}{!}{
%     \begin{tabularx}{300pt}{l@{\hskip .25in}c@{\hskip .4in}ccc}\toprule
%                                       & \multirow{2}{*}{\textbf{\gls{aflw}}}       & \multicolumn{3}{c}{\textbf{300W}}        \tabularnewline
%                                       &                             & \textbf{Common}        & \textbf{Challenge}   & \textbf{Full}              \\\midrule
                                      
% SDM~\cite{xiong2013supervised}            & 5.43                        & 5.57          & 15.40         & 7.52              \tabularnewline
% LBF~\cite{ren2014face}                    & 4.25                        & 4.95          & 11.98         & 6.32         		\tabularnewline
% MDM~\cite{trigeorgis2016mnemonic}         & -                           & 4.83          & 10.14         & 5.88         		\tabularnewline
% TCDCN~\cite{zhang2014facial}                & -                           & 4.80          & 8.60          & 5.54        		\tabularnewline
% CFSS~\cite{zhu2015face}                    & 3.92                        & 4.73          & 9.98          & 5.76         		\tabularnewline
% CFSS~\cite{lv2017deep}                     & 2.17                        & 4.36          & 7.56          & 4.99         		\tabularnewline
% RCSR~\cite{wang2018recurrentpami}          & -                           & 4.01          & 8.58          & 4.90         		\tabularnewline
% RCN+ (L$+$ELT)~\cite{honari2018improving}            & \textbf{1.59}               & 4.20          & 7.78          & 4.90         		\tabularnewline
% CPM $+$ SBR~\cite{dong2018supervision}            & 2.14                        & 3.28          & 7.58          & 4.10     	    	\tabularnewline\midrule
% $\Sam$                                & 2.26                        & 3.48          & 7.39          & 4.25    		    \tabularnewline
% $\Sam$+D(10K)                         & -                           & 3.34          & 7.90          & 4.23     		    \tabularnewline
% $\Sam$+D(30K)                         & -                           & 3.41          & 7.99          & 4.31     		    \tabularnewline
% $\Sam$+D(50K)                         & -                           & 3.41          & 8.06          & 4.32     		    \tabularnewline
% $\Sam$+D(70K)                         & -                           & 3.34          & 8.17          &  4.29     		    \tabularnewline\midrule
% $\lkl$                                & 1.97                        & 3.28          & 7.01          & 4.01     			\tabularnewline
% $\lkl$+D(10K)                         & -                           & 3.26          & 6.96          & 3.99            \tabularnewline
% $\lkl$+D(30K)                         & -                           & 3.29          & 6.74          & 3.96              \tabularnewline
% $\lkl$+D(50K)                         & -                           & 3.26          & \textbf{6.71} & 3.94              \\%\vspace{-3mm}
% $\lkl$+D(70K)                         & -                           & \textbf{3.19} & 6.87          & \textbf{3.91}     \\\bottomrule
%     \end{tabularx}
% %   }
% \end{table}

\begin{table}[t!]
\centering
\caption{\textbf{Quantitative results}. \gls{nmse} on \gls{aflw} and 300W normalized by the square root of BB area and interocular distance, respectfully.}
\label{tab:face-comparisons}
    
 \begin{tabular}{r|ccccc}%\toprule
     &\textbf{\gls{aflw}}&& \multicolumn{3}{c}{\textbf{300W}} \\
      &                 &            & \textbf{Common}        & \textbf{Challenge}   & \textbf{Full}              \\\midrule
     \cline{2}\cline{5-7}
SDM~\cite{xiong2013supervised}            & 5.43      &                  & 5.57          & 15.40         & 7.52              \tabularnewline
LBF~\cite{ren2014face}                    & 4.25       &                 & 4.95          & 11.98         & 6.32         		\tabularnewline
MDM~\cite{trigeorgis2016mnemonic}         & -           &                & 4.83          & 10.14         & 5.88         		\tabularnewline
TCDCN~\cite{zhang2014facial}                & -          &                 & 4.80          & 8.60          & 5.54        		\tabularnewline
CFSS~\cite{zhu2015face}                    & 3.92         &               & 4.73          & 9.98          & 5.76         		\tabularnewline
CFSS~\cite{lv2017deep}                     & 2.17          &              & 4.36          & 7.56          & 4.99         		\tabularnewline
RCSR~\cite{wang2018recurrentpami}          & -             &              & 4.01          & 8.58          & 4.90         		\tabularnewline
RCN+ (L$+$ELT)~\cite{honari2018improving}            & \textbf{1.59}    &           & 4.20          & 7.78          & 4.90         		\tabularnewline
CPM $+$ SBR~\cite{dong2018supervision}            & 2.14        &                & 3.28          & 7.58          & 4.10     	    	\tabularnewline\midrule
$\Sam$                                & 2.26                &        & 3.48          & 7.39          & 4.25    		    \tabularnewline
$\Sam$+D(10K)                         & -                    &       & 3.34          & 7.90          & 4.23     		    \tabularnewline
$\Sam$+D(30K)                         & -                   &        & 3.41          & 7.99          & 4.31     		    \tabularnewline
$\Sam$+D(50K)                         & -               &            & 3.41          & 8.06          & 4.32     		    \tabularnewline
$\Sam$+D(70K)                         & -               &            & 3.34          & 8.17          &  4.29     		    \tabularnewline\midrule
$\lkl$                                & 1.97            &            & 3.28          & 7.01          & 4.01     			\tabularnewline
$\lkl$+D(10K)                         & -               &            & 3.26          & 6.96          & 3.99            \tabularnewline
$\lkl$+D(30K)                         & -               &            & 3.29          & 6.74          & 3.96              \tabularnewline
$\lkl$+D(50K)                         & -               &            & 3.26          & \textbf{6.71} & 3.94              \\%\vspace{-3mm}
$\lkl$+D(70K)                         & -               &            & \textbf{3.19} & 6.87          & \textbf{3.91}     \\\bottomrule
%\bottomrule
\end{tabular}
\end{table}

==> tables/task2-results.tex <==
	\begin{tabular}{ccccccccccccc} 
         	  \multicolumn{13}{c}{Image} \tabularnewline \cline{2-12}
	 		&\multicolumn{5}{c}{Feature-level} && \multicolumn{5}{c}{Score-level} & \tabularnewline
		\cline{2-6}\cline{8-12}
		&mean	&median&	min&	max	&sum&&	mean	&median&	min	&max	&sum&Avg.\tabularnewline
		median	&87.7&	87.7&	82.0&	86.7&	87.7&&	87.8&	87.8&	82.1&	86.4&	87.8&	87.8\tabularnewline
		mean &88.7&	88.7&	82.9&	87.7&	88.7&&	88.3&	88.3&	82.9&	86.8&	88.3&	88.7\tabularnewline
		         	  \multicolumn{13}{c}{Video} \tabularnewline \cline{2-12}
\end{tabular} 

==> tex/5-Proposed-kin-models.tex <==
Automatic kinship recognition capability is relevant in awide range of practical case, with many whom reap benefit –such as consumers (e.g. automatic photo library managemen-t [33]), scholars (e.g. historic lineage & genealogical studies[3], [4]), analyzers (e.g. social-media-based analysis [14],[24], [9], [39]), and investigators (e.g. missing persons andhuman traffickers [25])– with advanced kinship recognitiontechnologies. Additionally, kinship is a powerful cue forautomatic understanding faces, and even the bigger picture of human-computer interaction as a whole, as the knowledgecould be used as high-level evidence in bigger problems,such as an attribute in conventional facial recognition. Fromthis, we are motivated to push the frontier of visual kinshiprecognition with the largest verification benchmarks forseveral types of relationships, running each with the dataneeded to properly represent that in the real-world (i.e.,from sources such as personal photo albums, social mediaoutlets, Hollywood, athletic associations, places of politicalpower, and many other unconstrained sources worldwide andin the wild). Amongst our top aspirations with this work is to attract more interest of researchers from the visionand related communities to help improve state-of-art and todesign new problems using the new large-scale database forkinship recognition (i.e.,Families in the Wild(FIW) [25]).This work is supported in part by the NSF IIP award 1635174 and ONRYoung Investigator Award N00014-14-1-0484.∗indicates equal contributions.Analogous to facial recognition, kinship recognition canbe viewed as a broader set of subtasks to tackle different practical purposes. Of these, kinship verification was the firstto be introduced back in 2010 [13]. But, even after the severalyears since then, automatic kinship recognition capabilityis still far from being mature enough to be employed inreal-world uses. We believe the reasons for the delay aresummarized in two-fold:1) Current kinship recognition datasets are insufficient in terms of size, diversity and, thus under represent actualfamily distributions in the real-world.2) Recognizing kinship in the visual domain is challenging, as there are hidden factors affecting the facialappearances amongst family members making for less discriminative power when compared to more conven-tional problems of its kind (e.g. facial recognition orobject classification).In response, we propose the largest benchmark for kinshipverification which involves several hundred thousand addi-tional pairs, opposed to just the couple of thousand thatwas available prior. We also achieve a significant boost inperformance using deep learning on this generous collectionof face pairs.Several methods were proposed for kinship verificationover the past decade. Of these attempts, there were several in-volving hand-crafted (i.e., low level) features (e.g. SIFT [18],LBP [1], PEM [17]), face encodings (e.g. fisher vectorsfaces [26]), and metric learning methods. The commonobjective of metric learning is to learn a good distancemetric to minimize distances between positive pairs, whilepushing pairs of different types further apart. Several rep-resentative metric learning algorithms have been applied tokinship verification, including neighborhood repulsed metriclearning (NRML) [20], large margin multi-metric learning(LM3L) [16], discriminative multi-metric learning (DMM-L) [36], and online similarity learning (OSL) [35].The goal of kinship verification is to determine whetheror not a pair of faces are related; opposed to conventionalfacial recognition where the task is to determine if a pairof faces are the same person. Existing metric learning ap-proaches only learn a linear transformation directly from theoriginal feature space to project the input samples into a newrepresentation, which may or may not be powerful enoughto explicitly capture the intrinsic structure hidden in kinshipknowledge, all awhile setting aside identity discrepancies and

==> tex/old-tex/4-FIW.tex <==
\chapter{FIW}
\section{Introduction}
My research is in applied machine vision with emphasis on automatic face and human body understanding in security, social context, and human-computer interaction. We built face and motion image and video collections to support these efforts. Most notably is the \gls{fiw}, which, by far, is the largest labeled image collection for automatic kinship recognition to date. Besides, focus has been set to improve facial landmark detectors using improved loss functions and machinery capable of leveraging unlabeled data to improve accuracy. These tracks (\ie work based on \gls{fiw} and facial landmark localization in settings where labeled data are scarce) are where most of the focus was spent and, thus, efforts that I led. Thus, independent sections of this proposal are dedicated to each one, with a summary of other contributions, both technical and professional, are merged into a section for completeness.
\begin{figure}[!t] 
	\centering    
	%\vspace{-7mm} 
	\begin{tabular}{ c | c | c } 
	%\begin{tabular}{ c  c  c } 
		%\multicolumn{1}{c}{\ }&\multicolumn{1}{c}{\  }&\multicolumn{1}{c}{ \ }\\
		\includegraphics[width=1.35in,height=3.25in, trim={.2mm 0mm 2mm 1mm},clip]{pairs_separate-3}&
		{\includegraphics[width=1.3in,height=3.25in, trim={0mm 0mm 1mm 1mm},clip]{pairs_separate-1}}&
	{\includegraphics[width=1.3in, height=3.25in, trim={0mm 0mm 0mm 1mm},clip]{pairs_separate-2}}\\ Same Generation &$1^{st}$ Generation &$2^{nd}$ Generation
	\end{tabular}
		\caption{\textbf{Samples of the $11$ pairwise types of \glspl{fiw}.} We show an unique pair randomly selected from a set of diverse families for each (\ie notice the diversity); also, the four faces of each individual were selected to span different ages to show the inherent age variant nature of the data. } \label{fig:pairs} 
\end{figure} 

This proposal is organized as follows. First the motivation, technical contributions, experiments, and concluding remarks are shared for the track concerning the \gls{fiw}. The same subtopics are next discussed for the semi-supervised facial landmark detector based on an improved loss function. Then, a summary of other research contributions are reviewed, which includes technical works, community services, and professional development. Finally, a conclusion is made with comments on future extensions and plans for the work presented throughout.

\section{Visual Kinship Recognition}

Visual kinship recognition has an abundance of practical uses, such as issues of human trafficking and in missing children, problems from today's refugee crises, and social media platforms. Use cases exist for the academic world as well, whether for machine vision (\eg reducing the search space in large-scale face retrieval) or a different field entirely (\eg historical \& genealogical lineage studies). However, to the best of our knowledge, no reliable system exists in practice. This is certainly not due to a lack of effort from researchers, as there are already many works focused on kin-based problems~\cite{ fang2013kinship,Xia201144, qin2015tri, duan2015neighbors, liu2015inheritable, chen2015kinship, chen2015sparse, duan2015feature,  vieira2014detecting, wang2014leveraging, xu2016kinship, yan2014discriminative, yan2015prototype, zhang2014talking, zhou2011kinship}. 

Challenges preventing visual kinship recognition from transitioning from research to reality are two-fold:

\begin{itemize}
\item Existing data resources for visual kinship are too small to capture true data distributions.
\item Hidden factors of visual similarities/differences between blood relatives are complex and less discriminant than in other more conventional problems (\eg object classification or even facial identification).
\end{itemize}





\begin{figure}[t!]
\centering
\includegraphics[width=\linewidth]{labeling.pdf}
   \caption{\textbf{Semi-automatic labeling pipeline.} \textit{Data Collection.} Photos and text metadata are collected for underrepresented families in \glspl{fiw} and assigned unique IDs (\ie PIDs). Each new member requires at least $1$ profile picture (\eg Brandon in $PID_1$) to add to known labels. \textit{Data Preparation.} With the existing \gls{fiw} labels, we next aim to increase the amount, both in labeled faces and member labels, using multiple modalities-- names in metadata and scores of \glspl{svm}s are used to automatically label some unlabeled data-- face-name pairs were assumed labeled for cases of high confidence. Starting from profile pictures (\ie 1 face, 1 name) and working towards less trivial scenarios (\eg 3 faces and 2 names, with 2 faces from 1 member at different ages, like in $PID_3$). This step adds to the amount of side information used for clustering \textit{Label Generation.}  Label proposals for remaining unlabeled faces are generated using the proposed semi-supervised clustering model that leverages labeled data as side information to better guide the process. \textit{Label Validation.} A GUI designed to validate clusters and ensure clusters are matched to the proper labels.} 
\label{fig:labeling_process}
\end{figure}


% \begin{figure}[!t] 
% 	\centering    
% 	%\vspace{-7mm} 
% 	\begin{tabular}{ c | c | c } 
% 	%\begin{tabular}{ c  c  c } 
% 		%\multicolumn{1}{c}{\ }&\multicolumn{1}{c}{\  }&\multicolumn{1}{c}{ \ }\\
% 		\subfloat[\footnotesize Same Generation]{\includegraphics[width=1.35in,height=3.5in, trim={.2mm 0mm 2mm 1mm},clip]{pairs_separate-3}\label{subfig:sib}}&
% 		\subfloat[$1^{st}$ Generation]{\includegraphics[width=1.3in,height=3.5in, trim={0mm 0mm 1mm 1mm},clip]{pairs_separate-1}\label{subfig:p-c}}&
% 		\subfloat[$2^{nd}$ Generation]{\includegraphics[width=1.3in, height=3.5in, trim={0mm 0mm 0mm 1mm},clip]{pairs_separate-2}\label{subfig:gp-gc}}
% 	\end{tabular}
% 		\caption{Samples of $11$ pair types of \glspl{fiw}. Each type is of a unique pair randomly selected from a set of diverse families to show variation in ethnicity, while four faces of each individual depict age variations. } \label{fig:pairs} 
% \end{figure} 


% (1) existing image datasets for kinship recognition are too small to capture the true data distributions of families worldwide and (2) visual evidence of kinship (\ie blood relationships) are less discriminant than in other, more conventional problems (\eg object classification or even conventional facial recognition). Thus, the hidden factors that highlight similarities and differences in the appearances of relatives are highly complex, varying greatly from one family to the next, and especially when considering diverse families. 


\begin{table*}\centering
	\caption {\textbf{Face pair~ counts for \glspl{fiw} and related databases.} \glspl{fiw} far outdoes all others in the $7$ \textit{sibling} \& \textit{parent-child} pair types. Plus, introduces $4$ \textit{grandparent-grandchild} types for the $1^{st}$ time. Fig. \ref{fig:pairs} shows samples for each pair type.}
	\ra{1.1}
	\scriptsize
	\begin{tabular}{@{}rccccccccccccccl@{}}\toprule
		& \multicolumn{3}{c}{{siblings}} & \phantom{a}& \multicolumn{4}{c}{{parent-child}} &
		\phantom{b} & \multicolumn{4}{c}{{grandparent-grandchild}}&
		 \multicolumn{1}{c}{Total}\\
		\cmidrule{2-4} \cmidrule{6-9} \cmidrule{11-14} 
		&BB & SS & SIBS&& FD & FS & MD & MS && GFGD & GFGS & GMGD & GMGS & \\\midrule
		KFW I~\cite{lu2014kinship}&0&0&0&&134&156 & 127 & 116 && 0 & 0 & 0 & 0 & 533 \\
		KFW II~\cite{lu2014kinship}&0&0&0&&250&250 & 250 &250 &&0&0&0&0 & 1,000 \\
		Group Face~\cite{guo2014graph}&40 &32 & 53 && 69&69 & 62 & 70 && 0 &0&0&0&395\\
			
	    SibFace~\cite{bottino2012new}& 232 & 211 &  277 &&0& 0&0&0&&0&0&0&0&720\\
%	Family 101~\cite{fang2013kinship}&0&0&0 && 147 &213 &148&184 &&0&0&0&0&& 607\\
%	FIW (Ours)~\cite{FIW}&\textbf{130,000}&\textbf{130,000} &\textbf{105,000} &\textbf{75,000}&\textbf{75,000} &\textbf{64,000} &\textbf{60,000}&\textbf{1,000}&\textbf{1,350}&\textbf{950}&\textbf{2,000}&\textbf{644,000} \\ 	\hline
\gls{fiw}(Ours)~\cite{FIW} &\textbf{103,724} &\textbf{39,978} & \textbf{73,506} &&\textbf{92,088} &\textbf{129,846}&\textbf{82,160} &\textbf{112,618}&&\textbf{7,078}&\textbf{4,830}&\textbf{6,512}& \textbf{4,614}&\textbf{656,954}\\
		\bottomrule
\end{tabular}
\label{tbl:pair_count1}
%\caption{Caption}
\end{table*}



Clearly, a large image-set that properly represents families worldwide is needed, which also meets the capacity of more complex, data-driven models (\ie deep learning), thus, motivating us to build the first large-scale image database for kinship recognition, \gls{fiw}.\footnote{More information and downloads on project-page, \url{https://web.northeastern.edu/smilelab/fiw/}} \glspl{fiw} is made-up of rich label information that captures the complex, hierarchical structures of 1,000 unique family trees. Families consist of an average of about 13 each (\ie over 13,000 family photos), and family sizes range from 3-38 members, with subjects having multiple samples at various ages. \glspl{fiw} is the \textbf{largest} and \textbf{most comprehensive} database of its kind.

Deep learning can now be applied to the problem, as we demonstrate on two benchmarks, kinship verification and family classification. We fine-tune deep models to improve all benchmarks, and provide details on the training procedure. 
% We also measure human performance to compare.



\begin{table}[t!]
\centering
\caption{\textbf{Comparison of \glspl{fiw} with related datasets.}}
 \scriptsize
 \centering
 \begin{tabular}{l*{2}{p{.85cm}<{\centering}}*{2}{p{.6cm}<{\centering}}{p{1.2cm}<{\centering}}} 
 % \begin{tabular}{l|p{.33in}p{.37in}p{.3in}p{.3in}p{.53in}}\hline
\toprule
 Dataset & No. Family & No. People &  No. Faces &  Age Varies & Family Trees \\ \midrule
 CornellKin\cite{fang2010towards} & 150  & 300 & 300 & \xmark & \xmark \\
 UBKinFace\cite{Ming_CVPR11_Genealogical,Xia201144}& 200 & 400 & 600 & \ 
\Large\checkmark 
& \xmark \\
 KFW-I\cite{lu2014neighborhood}& \xmark & 533 & 1,066 & $\xmark$ & \xmark\\
 KFW-II\cite{lu2014neighborhood}& \xmark & 1,000 & 2,000 & \xmark & \xmark \\
 TSKinFace\cite{qin2015tri} & 787 & 2,589 & \xmark & \Large\checkmark & \Large\checkmark \\
 Family101\cite{fang2013kinship} & 101 & 607 & 14,816 & \Large\checkmark & \Large\checkmark \\
 \gls{fiw}~\cite{FIW} & \textbf{1,000} & \textbf{10,676} & \textbf{30,725} & \Large\checkmark & \Large\checkmark\\
%  \multicolumn{1}{|>{\columncolor{mygray2}}l|}
%{FIW(Ours)~\cite{FIW}} & \multicolumn{1}{>{\columncolor{mygray2}}c}{\textbf{1,000}} & \multicolumn{1}{>{\columncolor{mygray2}}c}{\textbf{10,676}} & \multicolumn{1}{>{\columncolor{mygray2}}c}{\textbf{30,725}} & \multicolumn{1}{>{\columncolor{mygray2}}c}{\Large\checkmark} & \multicolumn{1}{>{\columncolor{mygray2}}c|}{\large\checkmark} \\
\bottomrule
\end{tabular} 
\label{tbl:compared}
\end{table}



We use a multimodal labeling model to optimize the annotation process. This includes a novel semi-supervised clustering method that works effectively in practice (\ie generates label proposals for new data using existing labeled data as side information). For this, we increase the amount of available side information using existing labels (\ie names), labeled faces, and text metadata collected with the family photos. We show a significant reduction in manual labor and time spent on labeling new data (see Fig. \ref{fig:labeling_process}).

We made a number of contributions with \gls{fiw}. Here listed are a few highlights:
%\cite{wen2016discriminative, kinFG2017}
\begin{enumerate}
\item Built the largest image set for kinship recognition to date. Then added additional faces for verification and complete families for classification. \gls{fiw} remains the largest public dataset in this domain.
%\item Mined labels via multi-modal approach.
%\item Proposed clustering algorithm and applied to generate label proposals.
\item Improved the labeling process with novel semi-supervised clustering method, which allowed us to drastically boost the size of \gls{fiw}.%, while increasing the amount of side-information for the algorithm via multi-modal mining pipeline.
\item Boosted baseline scores using novel deep learning approaches.
\item Obtained state-of-the-art on smaller, yet widely used, datasets via transferring CNN model fine-tuned on \gls{fiw}.
\item Conducted kinship verification experiment on humans and compared with algorithms.
\item Proposed generative model to predict the child from a pair of parents as input.
\item Held various data challenges to attract more researchers and, thus, push state-of-the-art.
\end{enumerate}


\subsection{Families In the Wild (FIW) Database}\label{sec:fw}
%We next cover the \glspl{fiw} database and method used to increase the amount of labeled data in semi-automatic fashion.
%%\footnote{Download FIW via project page, \url{smile-fiw.weebly.com/}.}
%
%
%\subsection{Overview}\label{subsec:existingfw}
Our goal was to collect and label about 10 family photos for 1,000 unique families. Labels are of 2 types, photo-level (\ie who is where in the image) and family-level (\ie all members present, and the relationships between one another).  The rich labels of \glspl{fiw} can serve as a resource for various types of vision tasks. For this, we benchmark the two popular tracks, kinship verification and family classification. Next, we introduce both tasks and the means of preparing the data.



%
%Even though it only took a small team to label 10,676 family photos and 1,000 families, the process relied heavily on human input. Plus, in the end, many families were not properly represented (\ie either too few members, face samples, or family photos). Thus, we aimed to reduce the manual labor and overall time requirements to add additional data and labels (i.e., for 61 existing families and 4 new replacements). Replacement families were those with too little data collected or available online. We next briefly describe how this was achieved.


%\subsection{Extending FIW}\label{subsec:extendingfw}
%The goal is to use the proposed semi-supervised model to generate label proposals for new data while using existing labels as side information to yield more accurate clusters. As explained in Section \ref{subsec:semi} and shown in Fig. \ref{fig:nmiplot}, the proposed clustering method only improves with more side information. Thus, we want to maximize the amount of side information (\ie labeled faces) available. We do this by inferring highly confident labels by aligning faces and names from the unlabeled photos and corresponding text metadata. In addition, and when available, we model labeled data to discriminate between family members in a photo. In the end, clusters are saved as ground truth upon being verified by a human. Significant savings, in manual labor and overall time, resulted from using this labeling process.

%A single family is processed at a time to reduce both the search and label spaces. We aim to discover labels with evidence from multiple modalities (\ie visual and contextual information). This not only increases the amount of side information available for clustering, but also the sample count to use for discovering more labels as face-name pairs. The cluster assignments (\ie label proposals) were then manually inspected (\ie validated).

%We demonstrate the effectiveness of the new labeling scheme by comparing the number of user inputs (\ie mouse clicks and keystrokes) and overall time with the process followed in \cite{FIW}. It took just a few inputs and a few minutes on average per family, opposed to hundreds of inputs and several minutes to over an hour (see Table \ref{tbl:compared}). \glspl{fiw} now contains a larger amount of data.

%faces of a particular family's photos with the target as label proposals for  individuals of the respective families. Resulting cluster assignments (or label proposals) are then manually inspected (\ie validated) generating ground-truth in an efficient manner. In the end, our new workflow proves to be significantly improved when compared to our previous approach. We demonstrate this comparing the two in terms of the number of user inputs (\ie mouse clicks and keystrokes) and amount of time-- results in just few inputs in the matter of a couple to a few minutes on average per family, which is down from hundreds of inputs in several minutes to over a hour (Table \ref{tbl:compared}). Additionally, FIW contains large amounts of new data and, moreover, $65$ families lacking proper representation have been extensively added to.
%made possible with the proposed clustering method that effectively labels in semi-supervised setting. 
%The end-to-end process is depicted in Fig. \ref{fig:labeling_process}, which we reference as 
%We next explain the improved multi-modal scheme as a four-step process: (1) \textit{Data Collection}, (2) \textit{Data Preparation}, (3) \textit{Label Generation}, and (4) \textit{Label Validation}. The goal of (1) and (2) is to prepare for clustering by gathering and increasing the side information available for (3), while (4) is to ensure correct label assignments for all newly collected data. In other words, we set out to increase the labeled sample pool (\ie side information) by inferring labels for unlabeled faces, which adds to the set of training exemplars. The faces that are still unlabeled in (3) are clustered using all labels as side information. All newly added data is then verified by a human. The process is illustrated in Fig. \ref{fig:labeling_process}, which we next describe step-by-step.


%\begin{figure}[b!]
%\centering
%\includegraphics[width=1\linewidth]{royaltree.pdf}
%   \caption{Cropped face samples of each member of British Royal Family included in FIW dataset (top).} 
%\label{fig:labeling_process}
%\end{figure}

%\noindent\textbf{Kinship verification} 
\paragraph{Kinship verification} Aims to determine whether two faces are blood relatives (\ie kin or non-kin). Prior research mainly focused on \textit{parent}-\textit{child} pairs (\ie father-daughter (F-D), father-son (F-S), mother-daughter (M-D), and mother-son (M-S)); some considered sibling pairs (\ie brother-brother (B-B), sister-sister (S-S), and brother-sister/mixed gender siblings (SIBS)). However, research in both psychology and computer vision revealed that different kin relations render different familial features, which motivated researchers to model different relationship types independently. With the existing image datasets used for kinship verification limited to, at most, 1,000 faces and typically only 4 relationship types, we believe such minimal data leads to overfitting and, hence, models that do not generalize well to unseen data captured \textit{in the wild}. \glspl{fiw} currently supports 11 relationship types, 4 being introduced to the research community for the first-time (\ie \textit{grandparent}-\textit{grandchild}) and, most importantly, each category is made up of many more pairs-- 418,000 face pairs in~\cite{FIW} has increased to 644,000 after extending \glspl{fiw} via the proposed semi-supervised approach. The 11 relationship types provide a more accurate representation for real-world scenarios. As mentioned, \glspl{fiw} is structured such that the labels can be parsed for different types of tasks and experiments, and additional kinship types can easily be inferred.


\paragraph{Family classification} Aims to determine the family an unknown subject belongs to. Families are modeled using the faces of all but one family member, with the member left out used for testing. This \textit{one-to-many} classification problem is a challenging problem that gets more challenging with more families. This is becuase families contain large intra-class variations that typically fool the feature extractors and classifiers, and each additional family further adds to the complexity of the problem. Additionally, and like conventional facial recognition, when the target is unconstrained faces \textit{in the wild} \cite{LFWTech} (\eg the variation in pose, illumination, expression, etc.), the problem continues to become more difficult. In~\cite{FIW}, the experiment included only 316 families (\ie families with $5+$ members). In this extended version, we now can include 524 families with the added data. We next present the process followed to extend \gls{fiw}. %Now there are $1,001$ families; moreover,  involved in the extended family classification experiments. 




\subsection{Discussion}
\gls{fiw} is the first large-scale dataset available for visual kinship recognition. We annotated complex hierarchical relationships with only a small team in a fast and efficient manner-- providing the largest labeled collection of family photos to-date.  \glspl{fiw} was structured to support multiple tasks with its dynamic label structure. We provided several benchmarks for kinship verification and family classification. Pre-trained CNNs were used as \textit{off-the-shelf} face encoders, which outperformed conventional methods. Results for both tasks were further improved by fine-tuning the CNN models on \glspl{fiw}. We measured human observers and compared their performance to the machine vision algorithms, showing that CNN models already surpass humans in recognizing kinship. We also hosted a couple a data challenges using \gls{fiw} to attract increased attention to the problem.\\
The size of \glspl{fiw}, along with the labels representing complex tree structures of $1,000$ families, makes it difficult to pinpoint the exact directions \glspl{fiw} will lead. Improving upon the benchmarks is one route, which is the focus of past, current, and future data challenges based on \glspl{fiw}. Also, additional task evaluations (\eg search \& retrieval and tri-subject), along with cross-discipline studies (\eg nature-based and human perception) are also promising directions.



One motivation of this survey is to establish cohesive views of the major milestones via protocols that are clearly defined, data splits that are ready for download, and trained models that make baselines reproducible.\footnote{\href{https://github.com/visionjo/pykinship}{https://github.com/visionjo/pykinship}} Hence, components to reproduce experiments that we report make up part of the supplemental material. We cover the edge cases that challenge \gls{sota}, including an examination of the different settings and training tricks that further our abilities in kin-based detection from faces.

